A Flexible Modeling Approach for Robust Multi-Lane Road Estimation

A robust estimation of road course and traffic lanes is an essential part of environment perception for next generations of Advanced Driver Assistance Systems and development of self-driving vehicles. In this paper, a flexible method for modeling multiple lanes in a vehicle in real time is presented. Information about traffic lanes, derived by cameras and other environmental sensors, that is represented as features, serves as input for an iterative expectation-maximization method to estimate a lane model. The generic and modular concept of the approach allows to freely choose the mathematical functions for the geometrical description of lanes. In addition to the current measurement data, the previously estimated result as well as additional constraints to reflect parallelism and continuity of traffic lanes, are considered in the optimization process. As evaluation of the lane estimation method, its performance is showcased using cubic splines for the geometric representation of lanes in simulated scenarios and measurements recorded using a development vehicle. In a comparison to ground truth data, robustness and precision of the lanes estimated up to a distance of 120 m are demonstrated. As a part of the environmental modeling, the presented method can be utilized for longitudinal and lateral control of autonomous vehicles.

==> ModelingProcess.tex <==
After elaborating on each individual step, the procedure leading to a lane model following the structure shown in~\ref{fig:architecture} is described in the following. The main part of the process consists of an iterative expectation maximization process that alternates between associating the input data to the current model and fitting a new model to the associated data.
\\
At the beginning of each algorithm loop, an initial model is needed for the first association. If a model was derived in the previous time step, it serves as initial guess after predicting it to the current time frame as described in~\ref{model-prediction}. If no previous model is available, the initial model is estimated based on the current input data (see section~\ref{lane-model-init}).During association of the input features to different lines of the current model, each line is extrapolated in longitudinal direction to also associate features that lie beyond the range of the previously derived model. After association, the scope of each lane model line and its attributes are determined based on the associated lane marking features. The range is given by the associated feature with the largest longitudinal distance and lane mark type, color and width~\footnote{The width attribute only distinguishes between narrow, wide and unknown but does not have a measured width value.} are determined using Dempster-Shafer theory. Possible parallelism of lines is determined based on their attributes. From a dashed narrow line one can conclude that it is parallel to its left and right neighboring lines. A continuous line on the other hand indicates lanes that separate into different directions and therefore no parallelism of lines beyond the continuous one is assumed.
\\
In the following maximization step all the information enters the fit as described in section~\ref{gauss-newton-fit}. The associated lane features are used for the measurement optimization and the lane model from the previous fit is used for time filter optimization to prevent large changes of the lane model between two time steps. Continuity of subsequent line segments and parallelism between lines is expressed as equality constraints. The fit yields a set of parameters representing a lane model. The new lane model is now used to again for association of the lane features and association and fit are iteratively repeated to obtain the optimal lane model for the present input data. The iterative process stops once there is no change in the association of features to lines in the lane model. To guarantee that new input data is processed immediately when available, an upper limit of five expectation maximization iterations is applied in practice. The resulting lane model for the current time step is defined by the parameters estimated in the last fit.

